Multimodal ArXiv: A Dataset for Improving Scientific Comprehension of Large Vision-Language Models

Large vision-language models (LVLMs) excel across diverse tasks involving concrete images from natural scenes. However, their ability to interpret abstract figures, such as geometry shapes and scientific plots, remains limited due to a scarcity of training datasets in scientific domains. To fill this gap, we introduce Multimodal ArXiv, consisting of ArXivCap and ArXivQA, for enhancing LVLMs scientific comprehension. ArXivCap is a figure-caption dataset comprising 6.4M images and 3.9M captions, sourced from 572K ArXiv papers spanning various scientific domains. Drawing from ArXivCap, we introduce ArXivQA, a question-answering dataset generated by prompting GPT-4V based on scientific figures. ArXivQA greatly enhances open-sourced LVLMs' mathematical reasoning capabilities, achieving a 10.4\% absolute accuracy gain on a multimodal mathematical reasoning benchmark. Furthermore, employing ArXivCap, we devise four vision-to-text tasks for benchmarking LVLMs. Evaluation results with state-of-the-art LVLMs underscore their struggle with the nuanced semantics of academic figures, while domain-specific training yields substantial performance gains. Our error analysis uncovers misinterpretations of visual context, recognition errors, and the production of overly simplified captions by current LVLMs, shedding light on future improvements.

==> figs/caption-statistic.tex <==
% Use figure* for multi-column figure

\begin{figure}[tp]
  \centering

  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/data-statistic/caption_lens_all.jpg}
    \caption{Chunk Caption Distribution.}
    \label{fig:subfig1}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/data-statistic/caption_lens.jpg}
    \caption{Main Caption Distribution.}
    \label{fig:subfig2}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/data-statistic/sub_caption_lens.jpg}
    \caption{Subcaption Distribution.}
    \label{fig:subfig2}
  \end{subfigure}

  \caption{Caption Statistic.}
  \label{fig:caption-statistic}
\end{figure}

==> figs/chunk-example.tex <==
% Use figure* for multi-column figure
\begin{figure}[!t]
    \centering
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/examples/1-1.png}
    \caption{Single Figure-Caption}
    \label{fig:subfig1}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/examples/1-2.png}
    \caption{Multiple Figure-Caption}
    \label{fig:subfig2}
  \end{subfigure}
  \caption{Chunk Example. \lilei{add case of arxiv qa}}
  \label{fig:chunk_example}
\end{figure}

==> figs/image-statistic.tex <==
% Use figure* for multi-column figure

\begin{figure}[tp]
  \centering
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/data-statistic/n_images_by_paper.jpg}
    \caption{Image Number Distribution over Paper.}
    \label{fig:subfig1}
  \end{subfigure}
  % \hfill
  % \begin{subfigure}{0.45\textwidth}
  %   \centering
  %   \includegraphics[width=\textwidth]{figs/data-statistic/n_images_by_block.jpg}
  %   \caption{Image Number Distribution over Block.}
  %   \label{fig:subfig2}
  % \end{subfigure}
  \hfill
  % \begin{subfigure}{0.45\textwidth}
  %   \centering
  %   \includegraphics[width=\textwidth]{figs/data-statistic/image_sizes.jpg}
  %   \caption{Image Size Distribution.}
  %   \label{fig:subfig2}
  % \end{subfigure}
  \caption{Image Statistic.}
  \label{fig:image-statistic}
\end{figure}

==> figs/title-abstract-statistic.tex <==
% Use figure* for multi-column figure

\begin{figure}[tp]
  \centering

  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/data-statistic/title_lens.jpg}
    \caption{Title Length Distribution.}
    \label{fig:subfig1}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/data-statistic/abstract_lens.jpg}
    \caption{Abstract Length Distribution.}
    \label{fig:subfig2}
  \end{subfigure}

  \caption{Title and Abstract Statistic.}
  \label{fig:title-abstract-statistic}
\end{figure}

==> figs/word_cloud.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/word_cloud.jpg}
    \caption{Wordcloud of our captions.}
    \label{fig:word-cloud}
\end{figure}


==> tables/statistics.tex <==
\begin{table}[tbh!]
    \centering
    \begin{tabular}{l|c}
    \toprule
       Field  & Total Number \\
       \midrule
       Title \& Abstract & 572,734 \\ 
       Image & 6,481,222 \\ 
       Caption & 3,961,133 \\ 
       \bottomrule
    \end{tabular}
    \caption{Data Statistics of the curated dataset.}
    \label{tab:data_statistics}
\end{table}

\begin{table}[tbh!]
    \centering
    \begin{tabular}{l|cc}
    \toprule
       Field  & Total Number & Word Number \\
       \midrule
       Block Caption & 3,963,576 & 193,482,743 \\ 
       Main Caption in Block & 3,958,840 & 188,590,156 \\ 
       Subcaption in Block & 1,025,704 & 4,892,587 \\ 
       \bottomrule
    \end{tabular}
    \caption{Caption Statistics of the curated dataset.}
    \label{tab:caption_statistics}
\end{table}


% \begin{table}[tbh!]
%     \centering
%     \begin{tabular}{l|cc}
%     \toprule
%        Field  & Statistic \\
%        \midrule
%        Image Number & 6,481,222 \\ 
%        Total Size & 892GB \\ 
%        \bottomrule
%     \end{tabular}
%     \caption{Image Statistics of the curated dataset.}
%     \label{tab:image_statistics}
% \end{table}


==> tables/transfer.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
        Model &  ScienceQA  \\
         &  \\ 
         
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
